Learning Fair Representations via an Adversarial Framework

Fairness has become a central issue for our research community as classification algorithms are adopted in societally critical domains such as recidivism prediction and loan approval. In this work, we consider the potential bias based on protected attributes (e.g., race and gender), and tackle this problem by learning latent representations of individuals that are statistically indistinguishable between protected groups while sufficiently preserving other information for classification. To do that, we develop a minimax adversarial framework with a generator to capture the data distribution and generate latent representations, and a critic to ensure that the distributions across different protected groups are similar. Our framework provides a theoretical guarantee with respect to statistical parity and individual fairness. Empirical results on four real-world datasets also show that the learned representation can effectively be used for classification tasks such as credit risk prediction while obstructing information related to protected groups, especially when removing protected attributes is not sufficient for fair classification.

==> discarded.tex <==

\subsection{Comparison to Previous Works}
\label{sec:comparison}
In this part, we compare the different between our adversarial framework to previous ones, especially that of~\citeauthor{edwards2015censoring} and ~\citeauthor{madras2018learning}.

To the best of our knowledge, previous works in adversarial learning for fairness is based on minimizing the performance of a classifier that predicts the protected attribute. In our language, they formulate the adversarial \emph{critic} as a classifier against the protected attribute. In relevant literature, it is also called an \emph{adversary}. 

The idea behind using a classifier as the critic is that if \textbf{any} classifier cannot predict the protected attribute, then the information is efficiently hidden, and the fairness condition can be met. \citeauthor{madras2018learning} designed a specific classification loss for the critic derived theoretical bounds for the statistical difference. 

However, using a classifier as the critic could problematic from an optimization prospective and in practice we found it tricky to tune.
In order for such adversarial framework to achieve theoretical bound of fairness, it has to ensure that \textbf{all} types of classifiers cannot predict the protected attribute. In practice, and in works of ~\citeauthor{edwards2015censoring} and~\citeauthor{madras2018learning}, they used fixed architecture for the adversary to predict the protected attribute. 
First, the adversary must be strong enough to ensure that the information about the protected attribute is hidden, and the balance between the complexity of the adversary and the encoder is tricky. When the encoder is too strong, it encodes sensitive information while the adversary is unaware. When the adversary is too strong, it will be hard for the encoder to worsen the performance of the adversary, and the performance of information preservation deteriorates too much. In either case, the information of the protected attribute might still be preserved. 
Finally, even when the adversary and the encoder achieves balance and the adversary cannot predict the protected attribute, one might always suspect that a stronger or a different model of classifier as the adversary can still predict the protected attribute. In short, to achieve the theoretical bounds for fairness, one has to try out all possible classifiers, which is impossible. 

Our work, however, reduces the statistical difference between different groups of the protected attribute \emph{directly}. It has several advantages. First, with our formulation, \textbf{any} classifier that satisfies the Lipschitz condition automatically yields fair results. Hence, we do not care much about the strength and architecture of the critic, as long as it is a good approximation of the Wasserstein distance. 
In our experiments, a linear critic and autoencoder is sufficient to ensure fairness for bivariate protected attributes and preserve other informations, while in traditional works which uses classifiers as the adversary, the structure of the autoencoder and the adversary is often much more complex. In practice, our model is much easier to tune and optimize. 
Finally, with our method being able to ensure the minimization of the statistical differences, \emph{individual fairness}, or consistency, can also be achieved. 


\begin{table}[t]
	\centering
	\resizebox{0.99\linewidth}{!}{
		\begin{tabular}{|l|l|c|c|c|c|c|}
			\hline
			Dataset                 & Method & K-S  &  F1   & Par.  & Con.  &  EMD  \\ \hline
			\multirow{6}*{Adult}    & Ori.   & 0.560 & 0.640 & 2.396 & 0.977 & 0.275 \\ %\cline{2-7}
			& AE     & 0.550 & 0.624 & 1.986 & 0.979 & 0.158 \\ %\cline{2-7}
			& Ori.-P & 0.550 & 0.620 & 1.953 & 0.979 & 0.182 \\% \cline{2-7}
			
			& AE-P   & 0.550 & 0.625 & 1.883 & 0.980 & 0.094 \\ %\cline{2-7}
			& LFR    & 0.310  &   0.485   & 1.267  & 0.759 &  0.068  \\% \cline{2-7}
			& NRL    & 0.464 & 0.579 & 1.052 & 0.987 & 0.015 \\ \hline
			\multirow{6}*{Statlog}  & Ori.   & 0.460 & 0.605 & 1.061 & 0.902 & 0.174 \\% \cline{2-7}
			& AE     & 0.466 & 0.608 & 1.067 & 0.901 & 0.018 \\% \cline{2-7}
			& Ori.-P & 0.462 & 0.607 & 1.040 & 0.903 & 0.170 \\ %\cline{2-7}
			
			& AE-P   & 0.454 & 0.604 & 1.042 & 0.901 & 0.012 \\% \cline{2-7}
			& LFR    & 0.220  & 0.426 & 1.027  & 0.881  & 0.039  \\% \cline{2-7}
			& NRL    & 0.368 & 0.557 & 1.017 & 0.959 & 0.005 \\ \hline
			\multirow{6}*{Fraud}    & Ori.   & 0.248  & 0.244  & 1.251  & 0.950  & 0.133  \\% \cline{2-7}
			& AE     & 0.237  & 0.242  & 1.342  & 0.950  & 0.341  \\% \cline{2-7}
			& Ori.-P & 0.244  & 0.244  & 1.007  & 0.952  & 0.115  \\ %\cline{2-7}
			& AE-P   & 0.233  & 0.240  & 1.004  & 0.952  & 0.364  \\% \cline{2-7}
			& LFR    & 0.025  & 0.192  & 1.059  & 0.798  & 0.049  \\% \cline{2-7}
			& NRL    & 0.232  & 0.238  & 1.039  & 0.955  & 0.027  \\ \hline
			\multirow{6}*{Investor} & Ori.   & 0.406  & 0.344 & 1.069 & 0.991 & 0.290 \\% \cline{2-7}
			& AE     & 0.393  & 0.340 & 1.126 & 0.992 & 0.112 \\ %\cline{2-7}
			& Ori.-P & 0.400 & 0.342  & 1.108 & 0.992 & 0.154 \\% \cline{2-7}
			
			& AE-P   & 0.380 & 0.335  & 1.102 & 0.992 & 0.112 \\% \cline{2-7}
			& LFR    & 0.272  & 0.278  & 1.098  & 0.851  & 0.026  \\% \cline{2-7}
			& NRL    & 0.391 & 0.336 & 1.011 &  0.997 & 0.027  \\ \hline
		\end{tabular}
	}
	\caption{Results on classification performance and fairness metrics. 
		\small K-S and F1 are evaluation metrics for classification. 
		%Higher values indicate better performance. 
		Par., Con., and EMD are indicators of fairness. Par. stands for statistical parity, and lower values (closer to one) suggests fairer prediction scores. Con. is short for consistency, where higher values (closer to one) indicates more individual fairness. EMD is the distribution difference between the two groups derived by the protected attribute. Lower values of EMD means that the corresponding features are more independent of the protected attribute. 
		Methods with higher K-S and F1, and lower Par., Con. and EMD perform better.  
		\normalsize }
	\vspace{-0.1in}
	\label{table:metric:cls}
\end{table}


==> sketch.tex <==
  \section{Theoretical Analysis}
\label{sec:theory}

This part is written to theoretically support our approach, by linking our approach (invalidating zemel2013learnings) and fairness ($t$-closeness, or the representation of protected group is not different from the unprotected.) \\ 

\begin{definition}
    $X\in \RR^d$ is the random variable. $Y$ is the random variable to be predicted by $X$. $f:\mathcal{X}\rightarrow\mathcal{Y}$ is a classifier. $\mathcal{L}(X, Y)$ is the set of all such functions (classifiers). $L(Y, f(X))$ gives the loss of $f$ over the sample $x$. 
    $x$ is a sample and $y$ is the corresponding random variable to be predicted.
\end{definition}

We assume that $Y$ takes only 0 or 1,$\prob(Y=1)= \prob(Y=0)$ and $L(y, f(x))=0$ if and only if $y=f(x)$. We further assume that $L(y,x) = L(x,y)$.

Normally we try to find $f=\argmin_{f}\expt[L(Y, f(X))] = \expt_X\expt_{Y|X}[L(Y,f(x))|X=x] $. We formalize the idea that any classifier fail to predict, and show that if it holds true, $X|Y=0$ and $X|Y=1$ follows the same distribution.

Construct a classifier $f^*(X)=1$ for all $x\in\RR^d$. This is the worst case scenario for a trained classifier, since it cannot obtain any additional information about $Y$ given $X$ to help make decision. 

\begin{definition}
    For any $f\in \mathcal{L}(X, Y)$, if
    \begin{equation}
        \expt[L(Y, f(X))| X\in G] \geq \expt[L(Y, f^*(X))| X\in G] \nonumber
    \end{equation}
    for all $G\subset \RR^d$.
    Then $f$ provides us with no useful information about $Y$. We say that $f$ is an invalidated classifier.
\end{definition}

\begin{theorem}
    If the above inequality holds for all $f \in \mathcal{L}(X, Y)$, i.e. all calssifiers are invalidated, clearly 
    \begin{eqnarray}
       \min_f\expt[L(Y, f(X))|X\in G] = \expt[L(Y, f^*(X))|X\in G] \label{eqn:thm:toprove} \\
        (G\subset \RR^d) \nonumber
    \end{eqnarray}
    When it happens, $\prob(X=x|Y=0) = \prob(X=x|Y=1)$ almost surely, if $\prob(Y=0)=\prob(Y=1)$.
\end{theorem}

\begin{proof}
   If the theorem doesn't hold, assume there is a subset $E\in\RR^d$ and $\prob(E)>0$ on which 
   \begin{eqnarray}
        & & \prob(X=x|Y=0) > \prob(X=x|Y=1), x\in E \nonumber \\
        & \Rightarrow & \prob(X\in E|Y=0) > \prob(X\in E|Y=1)
        \label{eqn:inq:1}
   \end{eqnarray}
   The direct consequence of \ref{eqn:inq:1} is 
   \begin{eqnarray}
        \prob(Y=0|X\in E) > \prob(Y=1|X\in E)
        \label{eqn:inq:2}
   \end{eqnarray}
   The assumption does not harm generality, because
If on the set $E, \prob(E)>0$, we have 
   \begin{equation}
    \prob(X=x|Y=0) < \prob(X=x|Y=1) \nonumber
   \end{equation}
   It leads to 
   \begin{eqnarray}
    & &\prob(X\in E|Y=0) < \prob(X\in E|Y=1) \nonumber \\ 
    &\Leftrightarrow & \prob(X\in \RR^d-E|Y=0) > \prob(X\in \RR^d-E|Y=1) \nonumber
   \end{eqnarray}
   Therefore there must be a subset $E'\subset \RR^d-E$ that satisfies $\prob(E')>0$ on which the inequality holds pointwise: $\prob(X=x|Y=0)>\prob(X=x|Y=1)$, $\forall x\in E'$. 

We already assumed that 
   \begin{equation}
    \prob(Y=0)=\prob(Y=1) 
    \label{eqn:inq:3}
   \end{equation} 

Estabilish a classifier $f_1\in\mathcal{L}(X, Y)$ s.t. when $x$ is given,
\begin{eqnarray}
    \prob(f_1(X)=0|X\in E) = 1
\label{eqn:inq:4}
\end{eqnarray} 
and $$ \prob(f_1(X)=1|X\notin E)=1 $$

Observe that $\expt[L(Y, f^*(X))] = L(0,1)\expt_X[Y=0|X]$,
Then
\begin{eqnarray}
     \expt[L(Y, f_1(X))] &  = & \expt_{Y|X}[L(Y, f_1(x))|X\in E]\prob(X\in E) +  \nonumber \\
    &  &\expt_{Y|X}[L(Y, f_1(x)|X\notin E)]\prob(X\notin E)
    \label{eqn:thm:total}
\end{eqnarray}

Since 
\begin{eqnarray}
    & & \expt_{Y|X}[L(Y, f_1(X))|X\in E] \nonumber \\
    & = & L(0,1)\prob(Y=1|X\in E) \nonumber \\
    & < & L(0,1) \prob(Y=0|X\in E) \nonumber \\ 
    & =  & \expt_{Y|X}[L(Y,f^*(X))|X\in E]
    \label{eqn:thm:term1}
\end{eqnarray}

And clearly 
\begin{eqnarray}
   \expt_X\expt_{Y|X} [L(Y, f_1(X))|X\notin E] = \expt_X\expt_{Y|X} [L(Y, f^*(X))|X\notin E]
   \label{eqn:thm:term2}
\end{eqnarray}

Combining \ref{eqn:thm:total}, \ref{eqn:thm:term1}, \ref{eqn:thm:term2}, we find that 
\begin{eqnarray}
     \expt[L(Y, f_1(X))] < \expt[L(Y, f^*(X))]
\end{eqnarray}
Which is a contradition to \ref{eqn:thm:toprove}.

The above proof shows that the set on which $P(Y=0|X=x)\neq P(Y=1|X=x)$ is of probability zero. 
\end{proof}
\normalsize

\begin{remark}
   The condition of the theorem, i.e. Eqn~\ref{eqn:thm:toprove}, describes the situation that any classifier, after training, cannot classify against $Y$.

   Therefore, to learn fair representation such that the value of $Y$ has no im pact on $X$, we only need to ensure that the representation invalidates any classifier against the protected variable.

   %The condition $\prob(Y=0)=\prob(Y=1)$ is crucial, suggesting that the representation should be learned on a distribution where it holds.
\end{remark}

\augment{If time allows, work out an approximate version.}
\hide{
We can further prove a approximate version of the theorem:

\begin{theorem}
    Suppose there is a $0<\delta<1/2$ s.t. 
    \begin{equation}
         \frac{\min_f\expt[L(Y,f(X))]}{\max_f{\expt[L(Y, f(X))]}} > 1-\delta
    \end{equation}
    Then 
\end{theorem}
}
